Message Scheduling for Performant, Many-Core Belief Propagation

Belief Propagation (BP) is a message-passing algorithm for approximate inference over Probabilistic Graphical Models (PGMs), finding many applications such as computer vision, error-correcting codes, and protein-folding. While general, the convergence and speed of the algorithm has limited its practical use on difficult inference problems. As an algorithm that is highly amenable to parallelization, many-core Graphical Processing Units (GPUs) could significantly improve BP performance. Improving BP through many-core systems is non-trivial: the scheduling of messages in the algorithm strongly affects performance. We present a study of message scheduling for BP on GPUs. We demonstrate that BP exhibits a tradeoff between speed and convergence based on parallelism and show that existing message schedulings are not able to utilize this tradeoff. To this end, we present a novel randomized message scheduling approach, Randomized BP (RnBP), which outperforms existing methods on the GPU.

==> Makefile <==
TOPLEVEL   := main.tex
TARGET     := main.pdf
DIFF_TARGET:= diff.pdf
ZIP_TARGET := 2019-hpec-arxiv.zip
TARGETS    := $(TARGET)
TARGETS    += $(DIFF_TARGET)
GREY_TARGETS:= $(TARGETS:%.pdf=%-grey.pdf)
COPY_TARGETS:= $(TARGETS:%.pdf=%-copy.pdf)
ZIP_DIR    := $(basename $(ZIP_TARGET))
MAKEFILES  := Makefile

DEPFILES   :=
DEPFILES   += $(wildcard *.sty)
DEPFILES   += $(wildcard *.cls)
DEPFILES   += $(wildcard *.bib)
DEPFILES   += $(wildcard *.bst)
DEPFILES   += $(wildcard *.tex)
DEPFILES   += $(wildcard *.pdf)
DEPFILES   += $(wildcard *.png)
DEPFILES   += $(wildcard *.py)
DEPFILES   += $(TOPLEVEL)
DEPFILES   += $(MAKEFILES)

GARBAGE    :=
GARBAGE    += comment.cut
GARBAGE    += $(TOPLEVEL:%.tex=%.log)
GARBAGE    += $(TOPLEVEL:%.tex=%.out)
GARBAGE    += $(TOPLEVEL:%.tex=%.aux)
GARBAGE    += $(TOPLEVEL:%.tex=%.dvi)
GARBAGE    += $(TOPLEVEL:%.tex=%.cb)
GARBAGE    += $(TOPLEVEL:%.tex=%.cb2)
GARBAGE    += $(TOPLEVEL:%.tex=%.bbl)
GARBAGE    += $(TOPLEVEL:%.tex=%.blg)
GARBAGE    += $(TOPLEVEL:%.tex=%.tdo)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.in)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.lua)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.out)
GARBAGE    += $(addprefix _markdown_,$(TOPLEVEL:%.tex=%))
GARBAGE    += $(addprefix _minted-,$(TOPLEVEL:%.tex=%))
GARBAGE    += $(wildcard figures/*-eps-converted-to.pdf)

# To use custom fonts, build with xelatex instead
LATEX      := pdflatex
LATEX      += -shell-escape
#LATEX       = xelatex
LATEXDIFF  := latexdiff --exclude-textcmd="section,subsection"

.PHONY: default
default: $(TARGET) $(TARGET:%.pdf=%-copy.pdf) $(TARGET:%.pdf=%-grey.pdf)

.PHONY: all
all: $(TARGETS) $(COPY_TARGETS) $(GREY_TARGETS) $(ZIP_TARGET)

$(TARGET): $(DEPFILES)

ECHO            := echo

# empty means it works, nonempty means it doesn't work
ESCAPE_WORKS    := $(shell $(ECHO) -e)
NEWLINE_WORKS   := $(shell $(ECHO) -n)

# A Makefile function
# @param 1: color (e.g., BLUE or GREEN)
# @param 2: message to be printed in the color
color_out_noline = \
             if [ -t 1 ] && [ -z "$(ESCAPE_WORKS)" ] && \
                [ -z "$(NEWLINE_WORKS)" ]; then \
               $(ECHO) -n -e "$(BASH_$1)$2$(BASH_CLEAR)"; \
             elif [ -z "$(NEWLINE_WORKS)" ]; then \
               $(ECHO) -n "$2"; \
             else \
               $(ECHO) "$2"; \
             fi
color_out = \
             if [ -t 1 ] && [ -z "$(ESCAPE_WORKS)" ]; then \
               $(ECHO) -e "$(BASH_$1)$2$(BASH_CLEAR)"; \
             else \
               $(ECHO) "$2"; \
             fi

BASH_CLEAR    := \e[0m
BASH_BLACK    := \e[0;30m
BASH_BROWN    := \e[0;33m
BASH_GRAY     := \e[0;37m
BASH_GREY     := \e[0;37m
BASH_DARKGRAY := \e[1;30m
BASH_DARKGREY := \e[1;30m
BASH_RED      := \e[1;31m
BASH_GREEN    := \e[1;32m
BASH_YELLOW   := \e[1;33m
BASH_BLUE     := \e[1;34m
BASH_PURPLE   := \e[1;35m
BASH_CYAN     := \e[1;36m
BASH_WHITE    := \e[1;37m

# print statistics of a tex file compilation
# @param $1: name of the log file
define TEX_STATS
	echo "$1 statistics:"
	echo "    ----"
	$(call color_out_noline,BLUE,  overfull:               )
	grep "^Overfull" $1 | wc -l
	$(call color_out_noline,BLUE,  underfull:              )
	grep "^Underfull" $1 | wc -l
	echo "    ----"
	$(call color_out_noline,BLUE,  total warnings:         )
	grep -i warning $1 | wc -l
	$(call color_out_noline,BLUE,  undefined citations:    )
	grep "Warning: Citation .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  undefined references:   )
	grep "Warning: Reference .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  duplicate labels:       )
	grep "Warning: Label .* multiply defined" $1 | wc -l
	echo "    ----"
	if [ "$$(type -P detex)" ]; then \
		$(call color_out_noline,BLUE,  total word count:       ); \
		detex $(1:%.log=%.tex) | wc -w; \
	  echo "    ----"; \
	fi
endef

%.pdf: %.tex
	@echo "$< -> $@"
	@$(LATEX) $< </dev/null >/dev/null || (tail -n 30 $*.log && false)
	@-bibtex $*  </dev/null >/dev/null
	@$(LATEX) $< </dev/null >/dev/null
	@$(LATEX) $< </dev/null >/dev/null
	@$(call TEX_STATS,$*.log)

%-copy.pdf: %.pdf
	@echo "$< -> $@"
	@cp $< $@

%-grey.pdf: %.pdf
	@echo "$< -> $@"
	@gs \
	  -sOutputFile="$@" \
	  -sDEVICE=pdfwrite \
	  -sColorConversionStrategy=Gray \
	  -dProcessColorModel=/DeviceGray \
	  -dCompatibilityLevel=1.4 \
	  -dNOPAUSE \
	  -dBATCH \
	  -q \
	  "$<"

images/%.eps: images/%.dot
	dot $< -Tps -o $@

images/%.ps: images/%.tex
	@echo "$< -> $@"
	@(cd images && $(LATEX) $(notdir $<)) </dev/null >/dev/null \
		|| (tail -n 30 $(<:%.tex=%.log) && false)

.PHONY: diff
diff: diff.pdf

diff.tex: old.tex new.tex
	@echo "old.tex + new.tex -> $@"
	@$(LATEXDIFF) old.tex new.tex 2>/dev/null > diff.tex

new.tex: latexpand $(DEPFILES)
	@echo "bisect.tex -> new.tex"
	@./latexpand --fatal --verbose --output new.tex bisect.tex 2>/dev/null

GARBAGE    += new.tex
GARBAGE    += diff.tex
TARGETS    += diff.pdf
GARBAGE    += old.log
GARBAGE    += old.out
GARBAGE    += old.aux
GARBAGE    += old.dvi
GARBAGE    += old.cb
GARBAGE    += old.cb2
GARBAGE    += old.bbl
GARBAGE    += old.blg
GARBAGE    += old.tdo
GARBAGE    += old.markdown.in
GARBAGE    += old.markdown.lua
GARBAGE    += old.markdown.out
GARBAGE    += old.pdf
GARBAGE    += new.log
GARBAGE    += new.out
GARBAGE    += new.aux
GARBAGE    += new.dvi
GARBAGE    += new.cb
GARBAGE    += new.cb2
GARBAGE    += new.bbl
GARBAGE    += new.blg
GARBAGE    += new.tdo
GARBAGE    += new.markdown.in
GARBAGE    += new.markdown.lua
GARBAGE    += new.markdown.out
GARBAGE    += new.pdf
GARBAGE    += new.tex
GARBAGE    += diff.log
GARBAGE    += diff.out
GARBAGE    += diff.aux
GARBAGE    += diff.dvi
GARBAGE    += diff.cb
GARBAGE    += diff.cb2
GARBAGE    += diff.bbl
GARBAGE    += diff.blg
GARBAGE    += diff.tdo
GARBAGE    += diff.markdown.in
GARBAGE    += diff.markdown.lua
GARBAGE    += diff.markdown.out
GARBAGE    += diff.tex

.PHONY: clean
clean:
	rm -rf $(GARBAGE)

.PHONY: veryclean
veryclean: clean
	rm -f $(TARGETS)
	rm -f $(COPY_TARGETS)
	rm -f $(GREY_TARGETS)
	rm -rf $(ZIP_DIR)
	rm -f $(ZIP_TARGET)

.PHONY: distclean
distclean: veryclean

.PHONY: zip
zip: $(ZIP_TARGET)

$(ZIP_DIR):
	@mkdir -p $(ZIP_DIR)

# @param 1: source file
# @param 2: destination directory
define COPY_TO_PATH
	mkdir -p $(strip $2)/$(strip $(dir $1))
	cp $1 $2/$1
	
endef

$(ZIP_TARGET): $(DEPFILES) | $(ZIP_DIR)
	@echo "copying files into $(ZIP_DIR)/"
	@$(foreach f,$(DEPFILES),$(call COPY_TO_PATH,$f,$(ZIP_DIR)))
	@echo "$(ZIP_DIR)/* -> $(ZIP_TARGET)"
	@zip -r $(ZIP_TARGET) $(ZIP_DIR) >/dev/null

